Exploring the higher-order QED effects on the differential distributions of Breit-Wheeler process in relativistic heavy-ion collisions

Extensive studies have been conducted in the past few decades to investigate potential signatures of higher-order QED effects in high-energy electromagnetic scattering processes. In our previous work, we have identified evidence of higher-order corrections in the total cross-section for the Breit-Wheeler process in relativistic heavy-ion collisions. However, the presence of higher-order QED corrections cannot be unambiguously proven solely based on total cross-section measurements due to substantial experimental and theoretical uncertainties. The objective of this paper is to explore the sensitivity of specific differential observables in the Breit-Wheeler process to higher-order QED effects in high-energy heavy-ion collisions. These investigations will provide guidance in determining the presence or absence of higher-order QED processes by conducting precise measurements in future experiments.

==> Observable.tex <==
\section{Event observable}
\label{observable}
\subsection{Differential cross-section}

\begin{figure*}[ht]
  \centering
  %\flushleft
  \subfloat[$\gamma \gamma \rightarrow e^+ e^-$ in Au+Au $\sqrt{s_{NN}}=200 $ GeV]{\includegraphics[width=0.33\linewidth]{RHIC_yield_e_v7_wAccnoTE.pdf}}
 %\hfill 	
  \subfloat[$\gamma \gamma \rightarrow \mu^+ \mu^-$ in Au+Au $\sqrt{s_{NN}}=200 $ GeV]{\includegraphics[width=0.33\linewidth]{RHIC_yield_mu_v7_wAccnoTE.pdf}}
 %\hfill
  \quad
  %\centering
  \subfloat[$\gamma \gamma \rightarrow e^+ e^-$ in Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV]{\includegraphics[width=0.33\linewidth]{LHC_yield_e_v7_wAccnoTE.pdf}}
 %\hfill 	
  \subfloat[$\gamma \gamma \rightarrow \mu^+ \mu^-$ in Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV]{\includegraphics[width=0.33\linewidth]{LHC_yield_mu_v7_wAccnoTE.pdf}}
  %\quad
  \subfloat[$\gamma \gamma \rightarrow \tau^+ \tau^-$ in Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV]{\includegraphics[width=0.33\linewidth]{LHC_yield_tau_v7_wAccnoTE.pdf}}
 \hfill
\caption{Differential cross section for the lowest order and higher order and their ratio calculated in impact parameter dependence for varied pair production with two beam configurations: Au+Au $\sqrt{s_{NN}}=200 $ GeV and Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV. Kinematic region is limited by the detector acceptance as described in Table.~\ref{table}.}
\label{yield}
\end{figure*}

In the original Bethe-Maximon theory, a significant correction to the total cross-section of pair production is predicted and has since been the focus of a series of dedicated work~\cite{Lee_2009,Hencken:1998hf,PhysRevLett.100.062302,BAUR20071}.
%The large columb correction to the total cross section of pair production is originally predicted in Bethe-Maximon theory and subsequently studied in a series of dedicated work~\cite{Lee_2009,Hencken:1998hf,PhysRevLett.100.062302,BAUR20071}. 
But this large correction has not been found in experimental measurements until two years ago by Zha and Tang~\cite{zha2021discovery}. They clarified the puzzle why the total cross-section correction had not been observed during previous long time as that the missing part of pair production within the geometrical radius of the nuclei compensates the negative higher-order correction. In the QED calculation, a product of photon propagators from two nuclei contributes directly to the matrix element. When two beams get close to each other with larger overlap, the correction ratio of the differential cross-section equal as the ratio of integration of photon propagator multiplication is intuitive to increase with a smaller impact parameter.

\begin{figure*}[ht]
  
  \centering
  %\flushleft
  \subfloat[$\gamma \gamma \rightarrow e^+ e^-$ in Au+Au $\sqrt{s_{NN}}=200 $ GeV]{\includegraphics[width=0.33\linewidth]{RHIC_t_e_v5.pdf}}
 %\hfill 	
  \subfloat[$\gamma \gamma \rightarrow \mu^+ \mu^-$ in Au+Au $\sqrt{s_{NN}}=200 $ GeV]{\includegraphics[width=0.33\linewidth]{RHIC_t_mu_v5.pdf}}
 %\hfill
  \quad
  %\centering
  \subfloat[$\gamma \gamma \rightarrow e^+ e^-$ in Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV]{\includegraphics[width=0.33\linewidth]{LHC_t_e_v5.pdf}}
 %\hfill 	
  \subfloat[$\gamma \gamma \rightarrow \mu^+ \mu^-$ in Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV]{\includegraphics[width=0.33\linewidth]{LHC_t_mu_v5.pdf}}
  %\quad
  \subfloat[$\gamma \gamma \rightarrow \tau^+ \tau^-$ in Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV]{\includegraphics[width=0.33\linewidth]{LHC_t_tau_v5.pdf}}
 \hfill
\caption{Spread in transverse momentum space for the lowest order and higher order and their ratio calculated in impact parameter dependence for varied pair production with two beam configurations: Au+Au $\sqrt{s_{NN}}=200 $ GeV and Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV.}
\label{t}
\end{figure*}

The observation of vacuum pair production is identified in ultra-peripheral collisions (UPC) with an impact parameter greater than twice the radius of the atomic nucleus ($b>2R_A$) to minimize hadronic background.
%In experiments, the observation of vacuum pair production is tagged in UPC ($b>2R_A$) to reject most of the hadronic background, and practically not enormous impact parameter due to the limited daughters transverse momenta. 
We calculate the total cross section as a function of impact parameter in Fig.~\ref{yield}.
%The calculation of total cross section is carried out in Fig.~\ref{yield} as a function of impact parameter. 
%The results show a consistently increasing ratio, starting with a sizable higher order effect at the unobservable small impact parameters. 
The results illustrate an increasing ratio, beginning with a significant higher-order effect at small impact parameters that cannot be detected.
It is intuitive to image an increment of higher-order impact on differential cross-section with large overlap. The ratio will gets progressively closer to one at further impact parameter. In addition, one can find no significant dependence of the daughter species to the sensitivity featured by the ratio. 
%The initial photon energy enhancement (larger $\gamma$) extents the shape of the ratio in the impact parameter phase, so the ratio of RHIC energy in b from 0 to 45(fm) resembles that of LHC in b from 0 to 55(fm). 
The initial photon energy enhancement (larger $\gamma$) extents the shape of the ratio in the impact parameter phase, making the ratio of RHIC energy in impact parameter range 0 to 45(fm) resemble that of the LHC in impact parameter range 0 to 55(fm).
%The electron pair generation has the largest cross section that can probably provide sufficient yield to reduce the uncertainty of the ratio in analysis. 
Further, electron pair generation has the largest cross-section and can reduce uncertainty in the analysis due to sufficient yield.

\begin{figure*}[ht]
  \centering
  \subfloat[$\gamma \gamma \rightarrow e^+ e^-$ in Au+Au $\sqrt{s_{NN}}=200 $ GeV]{\includegraphics[width=0.33\linewidth]{mass_e_60_80_paper.pdf}}
  \subfloat[$\gamma \gamma \rightarrow \mu^+ \mu^-$ in Au+Au $\sqrt{s_{NN}}=200 $ GeV]{\includegraphics[width=0.33\linewidth]{mass_mu_60_80_paper.pdf}}
\caption{Mass distribution for dielectron and dimuon pairs production in RHIC Au+Au $\sqrt{s_{NN}}$=200 GeV. No obvious dependence could be found as implied in expression for the differential cross section. Kinematic region is limited by the detector acceptance as described in Table.~\ref{table}.}
 \label{mass}
\end{figure*}


\subsection{Transverse momentum spectra}

The detection of the pair transverse momentum distribution spans the long history of the measurements of photon-induced processes. Low $P_{T}$ is a distinctive feature of vacuum pair production which indicates small virtuality since could be utilized as a effective tool to select a pure QED sample from hadronic background. As been confirmed in recent measurements in RHIC and LHC~\cite{adam2018low,ALICE:2022hvk}, a characteristic peak at low pair transverse momentum is discovered over the hadronic cocktail. On the other hand, a significant $P_{T}$ broadening effect has been found in RHIC and LHC peripheral collisions with relatively small impact parameter as what the projection in Fig.~\ref{t} tells us. It is indicated~\cite{Zha:2018tlq} that only the model with strong impact parameter dependence satisfactorily describes the effect. The impact parameter dependence of $P_{T}$ shape has also been studied and demonstrated in~\cite{STAR:2019wlg} so that the $\sqrt{\langle P_{T}^2 \rangle }$ which quantifies the spread of the transverse plane should be sensitive to high order effects. The first evidence of high order is found in $P_T$ distributions by Baltz~\cite{PhysRevLett.100.062302} under the theoretical model in light cone coordinate with the same regularized eikonal phase to estimate higher-order modification. In this study, we plot the $\sqrt{\langle P_{T}^2 \rangle }$ of lowest order and higher-order, along with the ratio, as a function of impact parameter in RHIC Au+Au $\sqrt{s_{NN}}$=200 GeV and LHC Pb+Pb $\sqrt{s_{NN}}$=5.02 TeV collisions. \newline




The $\sqrt{\langle P_{T}^2 \rangle }$ as the quadratic of the average of the momentum transfer is related to initial photon energy. An enhancement of the ratio is exhibited for LHC energy in comparison of RHIC. However, there is no significant higher-order contribution to $P_{T}$ broadening ($\approx10\%$), unlike the differential cross-section. In the same mass region, the $\sqrt{\langle P_{T}^2 \rangle }$ of $\mu^+\mu^-$ pair production has a flatter shape relative to that of the $e^+e^-$ pair production. Moreover, $\sqrt{\langle P_{T}^2 \rangle }$ gradually decreases with the increase of the impact parameter as the ratio rises first and then falls, forming a peak near 15 fm. The maximum location is not found to be affected by $\gamma$ and daughter mass. The particular peaks around 15 fm are slightly larger than two times nuclear radius where the strongest electromagnetic field is projected. The small discrepancy in the radii of the two nuclei does not lead to a clear variation in the peak location.\newline

In existing experiments, the precise measurements for $10\%$ discrepancy of very low pair transverse momentum are still challenging missions due to the uncertainty. 
To address non-perturbative QED in rigorous measurements of the $\sqrt{\langle P_{T}^2 \rangle }$ of the transverse momentum, more statistics and more peripheral samples are needed. Furthermore, the internal soft photon radiation is not currently incorporated in the calculation and requires further discussion.
%More statistics and more peripheral samples are expected to address non-perturbative QED in rigorous $\sqrt{\langle P_{T}^2 \rangle }$ measurements. The internal soft photon radiation is not incorporated in the calculation and needs to be in further discussion.%Moreover, the exact shape of the transverse momentum is extensively studied and the internal QED shower effect has been employed to describe notable tail in transverse momentum and acoplanarity distributions. 

\subsection{Lepton pair mass}


The invariant mass of the produced dilepton pair is also the virtuality of the initial photon-photon system. Due to the detector acceptance, the pair mass could only be measure at mass region over two times of the minimum transverse momentum cutoff of the daughter tracks. According to the QED description of the cross-section, there is no direct contribution of pair mass to the higher order correction. Analytically, the pair mass distributions should not be a sensitive probe to the higher order QED effects, displayed as the flat shape of calculation results in Fig.~\ref{mass}, 


\subsection{Azimuthal asymmetry amplitude}

Due to the fundamental quantum nature, the massless spin-1 particle photon has only two projected helicity state $J_{z} = \pm1$, while a virtual photon that carries a virtual mass could also locate at $J_{z} = 0$ state. During the interaction, the initial polarization of Weizsaeker-William (WW) photons transforms into angular momentum of the final electron-positron pair, so the total spin $J=2$ of initial photons system should be encoded in differential cross section. In consideration of spin interference effect, the predicted signatures are $\cos 2\phi$ and $\cos 4\phi$ modulation in the azimuthal angle $\phi$. The polarization angle $\phi$ is defined as the angle between $\vec{P}_{T} \equiv \vec{p}_{1T} + \vec{p}_{2T}$ and $\Delta \vec{P}_{T} \equiv \vec{p}_{1T} - \vec{p}_{2T}$, where $\vec{p}_{1T}$, $\vec{p}_{2T}$ are the transverse momentum of final state lepton respectively. \newline
Then the cross section could be written in a general form of:
\begin{equation}
f(\phi)=C\left(1+A_{2 \phi} \cos 2  \phi+A_{4  \phi} \cos 4 \phi\right),
\end{equation}
where C is a constant and $A_{2 \phi}$ ($A_{4  \phi}$) is the magnitude of $\cos 2  \phi$ ($\cos 4 \phi$). Then $A_{2 \phi}$ ($A_{4  \phi}$) can be equivalently calculated as two times of the average of $\cos 2  \phi$ ($\cos 4 \phi$) modulation,

\begin{equation}
A_{2 \phi} = \frac{2\int d\phi \cos 2\phi f(\phi)}{\int d\phi f(\phi)}, \quad A_{4 \phi} = \frac{2\int d\phi \cos 4\phi f(\phi)}{\int d\phi f(\phi)},
\end{equation}
which is extensively applied in experimental analysis.

The $A_{2 \phi}$ and $A_{4  \phi}$ of lowest order and higher-order are presented for each beam set and pair species in Fig.~\ref{Aphi}. The highest modification factors of higher-order are shown to be around 15 fm, which is same as $\sqrt{\langle P_{T}^2 \rangle }$. The shapes of higher-order and lowest order ratio remain similar below b=2R  for both RHIC and LHC. The large lorentz boost factor allows the electromagnetic field to spread farther, resulting in a slower degradation of the photon density in transverse spatial phases in UPCs, reflected in the ratio. In contrast to the differential cross section, the ratio of $A_{4  \phi}$ in RHIC rapidly converges to unity as the collision parameter increases. An obvious sign transition is found in the lowest-order $A_{2 \phi}$ but not in higher-order calculations, so the ratio of $A_{2 \phi}$ propose a powerful probe for higher-order QED phenomenon. The random fluctuations observed in the ratio at large impact parameters in LHC muon and tau pair production are attributed to the exponential term $\exp \left(iq_{1\perp}b\right)$.

\begin{figure*}[ht]
  \centering
  \subfloat[$A_{4 \phi}$ for $\gamma \gamma \rightarrow e^+ e^-$ in Au+Au 200 GeV]{\includegraphics[width=0.33\linewidth]{RHIC_A4phi_e_v7_bin.pdf}}
  \subfloat[$A_{4 \phi}$ for $\gamma \gamma \rightarrow \mu^+ \mu^-$ in Au+Au 200 GeV]{\includegraphics[width=0.33\linewidth]{RHIC_A4phi_mu_v7_bin.pdf}}
  %\centering
  \subfloat[$A_{2 \phi}$ for $\gamma \gamma \rightarrow \mu^+ \mu^-$ in Au+Au 200 GeV]{\includegraphics[width=0.33\linewidth]{RHIC_A2phi_mu_v7.pdf}}
 %\hfill 	
  \quad
  %\subfloat[img 4]{\includegraphics[width=0.33\linewidth]{LHC_A4phi_e_v7_bin.pdf}}
  \subfloat[$A_{4 \phi}$ for $\gamma \gamma \rightarrow e^+ e^-$ in Pb+Pb 5.02 TeV]{\includegraphics[width=0.33\linewidth]{LHC_A4phi_e_v7_bin.pdf}}
  \subfloat[$A_{4 \phi}$ for $\gamma \gamma \rightarrow \mu^+ \mu^-$ in Pb+Pb 5.02 TeV]{\includegraphics[width=0.33\linewidth]{LHC_A4phi_mu_v7_bin.pdf}}
  \subfloat[$A_{2 \phi}$ for $\gamma \gamma \rightarrow \tau^+ \tau^-$ in Pb+Pb 5.02 TeV]{\includegraphics[width=0.33\linewidth]{LHC_A2phi_tau_v7.pdf}}
  %\quad
\caption{Amplitudes of 2th and 4th modulation in final state $\phi$ distribution due to the initial photon linear polarization. The lowest order and higher order and their ratio calculated in impact parameter dependence for varied pair production with two beam configurations: Au+Au $\sqrt{s_{NN}}=200 $ GeV and Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV. Kinematic region is limited by the detector acceptance as described in Table.~\ref{table}.}
 \label{Aphi}
\end{figure*}

Following the relationship of lowest order $A_{2\phi}$, $A_{4\phi}$ with the lepton mass m and $\Delta P_{T}$ in the more modern model~\cite{Li:2019yzy} as

\begin{equation}
\begin{aligned}
& A_{2\phi} \propto \frac{4 m^2 \Delta P_{T}^2}{\left(m^2+\Delta P_{T}^2\right)^2} \sim \frac{4 m^2}{\Delta P_{T}^2}, \quad(\Delta P_{T}^2 \gg m); \quad  \\
& A_{4\phi} \propto \frac{- 2 \Delta P_{T}^4} {\left(m^2+\Delta P_{T}^2\right)^2} \sim -2(1-\frac{m^2}{\Delta P_{T}^2}), \quad(\Delta P_{T}^2 \gg m),
\end{aligned}
\end{equation}
%it could be inferred analytically that higher-order QED prefers larger $A_{4\phi}$ and smaller $A_{2\phi}$ than the lowest order due to the rise of $\Delta P_{T}$. According to this relationship, 
It is analytically inferred that higher-order QED prefers $A_{4\phi}$ with a larger value and $A_{2\phi}$ with a smaller value than the lowest order, due to the increase of $\Delta P_{T}$. Based on this relationship, the $A_{2 \phi}$ of electron pair production in RHIC (LHC) and muon pair production in LHC are negligibly small so that they are hardly be precisely measured and not presented in results.



%(. It was only recently realized that these effects could be accessed experimentally in ultrarelativistic heavy-ion collisions [9]
%since the transverse momentum of the pair is correlated with the polarization of the photons.)

==> Theoretical.tex <==
%\section{QED approach to the cross section}

\section{Theoretical framework}
\label{theo}
\subsection{Lowest order QED}



The lowest order cross section of pair production was first studied by Landau and Lifshitz~\cite{Landau:1934zj} and Racah~\cite{racah1937sulla}. The fast-moving heavy-ions are assumed with constant velocity along straight trajectory and small deflections due to the collisions are neglected. The electromagnetic fields carried by nuclei are treated  as external, which reads

\begin{equation}
A_\mu^{(1,2)}(q)=-2 \pi Z e u_\mu^{(1,2)} \delta\left(q u^{(1,2)}\right) \frac{f\left(q^2\right)}{q^2} \exp (\pm \mathrm{iqb} / 2)
\end{equation}
where $u^{(1,2)}$ is the four-velocity of ion 1 and 2 with electric charge Z and b is the impact parameter. The form factor $f(q^2)$ is Fourier transform of nuclear charge distribution. Wood-Saxon distribution is generally utilized to describe the charge distribution of heavy ion,

\begin{equation}
\rho_A(r)=\frac{\rho^0}{1+\exp \left[\left(r-R_{\mathrm{WS}}\right) / d\right]}
\end{equation}
where $\rho^0$ is the normalization factor, $R_{WS}$ and d are parameters of radius and skin depth. In this paper, Yukawa potential is employed to closely reproduce the form factor from
Fourier transform of the Wood-Saxon distribution, so we get

\begin{equation}
f(q)=\frac{3}{(q r)^3}[\sin (q r)-q r \cos (q r)]\left[\frac{1}{1+a^2 q^2}\right],
\end{equation}
where potential range $a = 0.7 fm$. The four-velocity of nuclei can be written as $u^{(1,2)}(q)=\gamma(1,0,0, \pm \beta)=: \gamma \omega^{(1,2)}$ in center of mass frame. Two Feynman diagrams contribute to pair creation through photon photon fusion as Fig.~\ref{feynman}. The matrix element of BH process is given by
\begin{equation}
M=\bar{u}\left(p_{-}\right) \hat{M} v\left(p_{+}\right).    
\end{equation}
%with

%\begin{strip}
%\begin{equation}
%\begin{aligned}
%\hat{M}%= & -i e^2 \int \frac{d^4 q_1}{(2 \pi)^4} A^{(1)}\left(q_1\right) \frac{\not p_{-}-\not q_1+m}{\left(p_{-}-q_1\right)^2-m^2} A^{(2)}\left(p_{+}+p_{-}-q_1\right) \\
%& -i e^2 \int \frac{d^4 q_1}{(2 \pi)^4} A^{(2)}\left(p_{+}+p_{-}-q_1\right) \frac{q_1-\slashed{p}_{+}+m}{\left(q_1-p_{+}\right)^2-m^2} A^{(1)}\left(q_1\right) \\
%= & -i\left(\frac{Z e^2}{2 \pi}\right)^2 \frac{1}{2 \beta} \int d^2 q_{1 \perp} \frac{1}{q_1^2} \frac{1}{\left(p_{+}+p_{-}-q_1\right)^2} \exp \left(iq_{1 \perp} b\right) \\
%& \left\{\frac{\slashed{\omega}^{(1)}\left(\slashed{p}_{-}-\slashed{q}_1+m\right) \slashed{\omega}^{(2)}}{\left[\left(p_{-}-q_1\right)^2-m^2\right]}+\frac{\slashed{\omega}^{(2)}\left(\slashed{q}_1-\slashed{p}_{+}+m\right) \slashed{\omega}^{(1)}}{\left[\left(q_1-p_{+}\right)^2-m^2\right]}\right\}.
%\end{aligned}
%\end{equation}
%\end{strip}

%where 
The energy and longitude momentum of one emitted photon can be expressed as $q_{10}=\frac{1}{2}\left[\left(\epsilon_{+}+\epsilon_{-}\right)+\beta\left(p_{+z}+p_{-z}\right)\right]$ and $q_{1 z}=q_{10} / \beta$. The $\epsilon$ and m are the energy and the mass of produced leptons.
Then it is straightforward to calculate the probability of the lowest order pair creation as:


\begin{strip}
\begin{equation}
\begin{aligned}
P\left(p_{+}, p_{-}, b\right)=\sum_s|M|^2= & \frac{4}{\beta^2} \int d^2 q_{1 \perp} d^2 \Delta q_{\perp} \exp \left(\mathrm{i \Delta q}_{\perp} \mathrm{b}\right) \\
& \times f\left(N_0\right) f\left(N_1\right) f\left(N_3\right) f\left(N_4\right) F\left(N_0\right) F\left(N_1\right) F\left(N_3\right) F\left(N_4\right) \\
& \times \operatorname{Tr}\left\{\left(\slashed{p}_{-}+m\right)\left[N_{2 D}^{-1} \slashed{\omega}_1\left(\slashed{p}_{-}-\slashed{q}_1+m\right) \slashed{\omega}_2+N_{2 X}^{-1} \slashed{\omega}_2\left(\slashed{q}_1-\slashed{ p}_{+}+m\right) \slashed{\omega}_1\right]\right. \\
& \left.\left(\slashed{p}_{+}-m\right)\left[N_{5 D}^{-1} \slashed{\omega}_2\left(\slashed{p}_{-}-\slashed{q}_1-\slashed{q}+m\right) \slashed{\omega}_1+N_{5 X}^{-1} \slashed{\omega}_1\left(\slashed{q}_1+\slashed{q}_1-\slashed{p}_{+}+m\right) \slashed{\omega}_2\right]\right\},
\end{aligned}
\end{equation}
\end{strip}

where integration variable $\Delta q_{\perp}$ is defined as the transverse projection of $\Delta q \equiv q_{1} -q_{1}^{\prime}$, with

\begin{equation}
\begin{aligned}
N_0 & =-q_1^2, \quad N_1=-\left[q_1-\left(p_{+}+p_{-}\right)\right]^2, \\
N_3 & =-\left(q_1+\Delta q\right)^2,\quad N_4=-\left[\Delta q+\left(q_1-p_{+}-p_{-}\right)\right]^2, \\
N_{2 D} & =-\left(q_1-p_{-}\right)^2+m^2, \\
N_{2 X} & =-\left(q_1-p_{+}\right)^2+m^2, \\
N_{5 D} & =-\left(q_1+\Delta q-p_{-}\right)^2+m^2, \\
N_{5 X} & =-\left(q_1+\Delta q-p_{+}\right)^2+m^2,
\end{aligned}    
\end{equation}
The photon propagator $F\left(N_k\right)$ for perturbative Columb interaction in the limit $Z\alpha \rightarrow 0$ is given by

\begin{equation}
F\left(N_k\right)=\frac{Z \alpha}{N_k}=\frac{Z \alpha}{\frac{\omega_k^2}{\gamma^2}+p_{T k}^2}, \quad k=0,1,3,4
\end{equation}
where $\alpha$ is the fine structure constant. The limitation of $Z\alpha$ makes higher order ($>2$) of $o(Z\alpha)$ negligible, so it represents the lowest order perturbative QED case. The impact parameter b dependence of the probability is calculated as the integration over 6-dimensional momentum space of the lepton pair
\begin{equation}
P_{\text {total }}\left(b\right)=\int \frac{d^3 p_{-} d^3 p_{+}}{(2 \pi)^6 2 \epsilon_{-} 2 \epsilon_{+}} P\left(p_{+}, p_{-}, b\right).
\end{equation}
Through further integration over the impact parameter, we get the total cross section as

\begin{table*}%[H]
\caption{\textbf{Detector acceptance implemented in the calculation}}
\centering
\begin{tabular}{llccccc}
\toprule
\multicolumn{2}{c}{Process and beam energy} & $p_{Tl}$ (GeV)& $\eta_{l}$ & $P_{Tll}$ (GeV) &$Y_{ll}$ & $M_{ll}$ (GeV)\\
\midrule
$\gamma \gamma \rightarrow e^+ e^-(\mu^+ \mu^-)$ &Au+Au $\sqrt{s_{NN}}=200 $ GeV & $(0.2,+\infty)$& $(-1.0,1.0)$& $(0,0.3)$& $(-1.0,1.0)$& $(0.4,2.6)$\\
$\gamma \gamma \rightarrow e^+ e^-$ &Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV& $(0.5,+\infty)$& $(-1.0,1.0)$& $(0,0.3)$&  $(-1.0,1.0)$ &$(1.0,2.8)$\\
$\gamma \gamma \rightarrow \mu^+ \mu^- (\tau^+ \tau^-)$ &Pb+Pb $\sqrt{s_{NN}}=5.02$ TeV & $(4.0,+\infty)$& $(-2.4,2.4)$& $(0,0.3)$& $(-2.4,2.4)$ & $(8.0,100.0)$\\
\bottomrule
\end{tabular}
\label{table}
\end{table*}


\begin{equation}
\sigma_{\text {total }}=\int d^2 b P_{\text {total }}(b).
\end{equation}
In this QED approach, the possibility expressed as impact parameter dependence can be expended to small b. The oscillating phase $\exp \left(\mathrm{i \Delta q}_{\perp} \mathrm{b}\right)$ involved in the integral over the difference of $q_1$ and $q_1^{\prime}$ presents a numerical challenge to the cross section calculation for the large impact parameter. 
%A series of solution have been proposed to deal with it. 
However, higher order corrections are not predicted to be significant at large b within experimental limited phase space. So impact parameter is considered to be limited under 45 (55) fm in calculation, which is a numerical more treatable case.

This paper performs calculations to quantify the sensitivities of differential cross-section, $A_{2\phi}$ ($A_{4\phi}$) and $\sqrt{\langle P_{T}^2 \rangle }$ to higher-order effects in impact parameter dependence in RHIC (LHC) energies. 

\subsection{Higher-order QED corrections}

The theoretical study of higher-order effect is pioneered by the Bethe and Maximon’s seminal work~\cite{PhysRev.93.768}. Ivanov, Schiller, and Serbo pointed out~\cite{Ivanov:1998ru} that a negative (Coulomb) correction ($\propto Z^2$) to the total cross section of pair production was described in the Bethe-Maximon theory, which is contrary to the well known fact. The Furry-Sommerfeld-Maue wave function as solution of Schrodinger equation was derived in Bethe and Maximon’s work. Lee and Milstein later noted~\cite{Lee:1999eya,Lee:2001nt} that the screening Columb potential should be used for regularization in transverse spacial space, and suggested the eikonal phase as the modified Bessel function 

\begin{equation}
\chi(\rho)=-2 Z \alpha K_0\left(\rho \omega / \gamma\right),
\end{equation}
where $K_0(\rho \omega / \gamma)=-\ln (\rho)-\ln (\omega / 2 \gamma)-\gamma_e$ has the physical cutoff $\rho \approx \gamma / \omega$. The proper expression of the modified photon propagator is given by

\begin{equation}
F(\mathbf{k})=  2 \pi \int d \rho \rho J_0(k \rho) \left\{\exp \left[2 i Z \alpha K_0\left(\rho \omega / \gamma\right)\right]-1\right\},
\label{HOFF}
\end{equation}
which goes to the familiar lowest order form $F^0(k)=4 \pi i Z \alpha /(k^2+\omega^2 / \gamma^2)$ in the perturbative limit $Z \alpha \rightarrow 0$. In our calculations, Eq.~(\ref{HOFF}) is utilized for higher order correction.

The trigger efficiency of no hadronic interaction and Coulomb dissociation have not been considered in this theoretical framework. They will compensate the higher order correction at some extend in peripheral collisions, like 60-80\% centrality, but negligible in UPCs.


\subsection{Fiducial experimental acceptance employed in integration}
Due to the detector acceptance, a good quality track of daughter lepton is defined in a fiducial phase space with a minimum transverse momentum cutoff within a specific pseudo-rapidity region. 
The cross-section of exclusive lepton pair production is therefore naturally measured at large pair invariant mass and small pair transverse momentum so as to ensure a low photon virtuality.
%Thus, the cross-section of exclusive lepton pair production is naturally measured at large pair invariant mass and small pair transverse momentum to ensure the low photon virtuality. 
The detailed configuration utilized in the integration is listed in Table.~\ref{table}. 
Higher-order effects on selected event observables within the fiducial kinematic regions are quantified by determining the ratio of values obtained from higher-order and lowest order calculations, as detailed in Sec.~\ref{observable}.
%Within the fiducial kinematic regions, the impact of higher-order effects on the selected event observables are quantified by the ratio of values from higher-order calculation and lowest order results, detailed in Sec.~\ref{observable}.

In addition to UPCs, the measurements of photon photon production of lepton pair are found occur even with hadronic overlap. 
Separating the electron-positron pair from other processes can be challenging in high-energy collisions. The detector system's excellent electron identification allows for the exclusive photo-produced lepton pair to be isolated from hadronic interactions based on a feature that concentrates at very low transverse momentum within a specific mass range.
%In high-energy collisions, it seems a challenging task to separate the electron positron pair from other processes. With the excellent electron identification of the detector system, the exclusive photo-produced lepton pair is qualified to be isolated from hadronic interaction by the feature concentrating at very low transverse momentum over a specific mass range. 
However, this could only be in mid-central collisions as the overabundant pairs from hadronic interactions would swamp those from photoproduction in more central collisions. 
% at ATLAS  b can reach 0  but not exclusive production
%The excellent electron identification of detector system and  qualified to 
% we'd like to write the reason of choosing such large pair mass region here, like what is said in report of progress... (the last paragraph at P50)

%\begin{table}%[H]
%\caption{\textbf{Acceptance applied in the calculation}}
%
%\begin{tabular}{llccccc}
%\toprule
%\multicolumn{2}{c}{Process and beam energy} & $p_{Tl}$ (GeV)& $\eta_{l}$ & %$P_{Tll}$ (GeV) &$Y_{ll}$ & $M_{ll}$ (GeV)\\
%\midrule
%$\gamma \gamma \rightarrow e^+ e^-(\mu^+ \mu^-)$ &Au+Au $\sqrt{s_{NN}}=200 %$ GeV & $0.2<p_{Tl}$& $\lvert \eta_{l} \rvert <1.0$& $P_{Tll}<0.3$& $\lvert %Y_{ll} \rvert <1.0$& $0.4<M_{ll}<2.6$\\
%$\gamma \gamma \rightarrow e^+ e^-$ &Pb+Pb $\sqrt{s_{NN}}=5.02 $ TeV& $0.5<p_{Tl}$& $\lvert \eta_{l} \rvert <1.0$& $P_{Tll}<0.3$&  $\lvert Y_{ll} \rvert <1.0$ &$1.0<M_{ll}<2.8$\\
%$\gamma \gamma \rightarrow \mu^+ \mu^- (\tau^+ \tau^-)$ &Pb+Pb $\sqrt{s_{NN}}=5.02$ TeV & $4.0<p_{Tl}$& $\lvert \eta_{l} \rvert <2.4$& $P_{Tll}<0.3$& $\lvert Y_{ll} \rvert < 2.4$ & $8.0<M_{ll}<100.0$\\
%\bottomrule
%\end{tabular}
%\end{table}




%Higher-order effect has been a subject of intensive study in the last few decades and recent experimental evidence reveals that non-perturbative QED effect is possible to be detected in HIC.


%Although Coulomb correction is undoubtedly proven to exist in real physical processes, the inconsistency of the experimental results has not been conclusively established until now. Therefore more and stronger evidence of higher order effects is expected to be found in the analysis of large statistical data. The question about what observables are sensitive to higher order effects and may provide strong signals is important for the analysis of experimental data. In this paper, the sensitivity of selected observables and higher-order effects is studied from a theoretical point of view to suggest a valid path.


%unambiguous (明确的)

==> readme.tex <==
figures needs to be updated,
put them here to have a direct view of the format
Question: Why use NIMA template? -- Zebo
A: It is actually standard elsevier backage, ``preprint to NIMA" should be commented out. On the other hand, one column is applied to the article while two columns format is widely used in NIMA.  -my point of view...
Q: No problem. So the target journal is Phys. Lett. B? 
A: I hope so, while it needs a discussion.
C: One column is usually for preprint and two column is commonly used in the final production. Remember to use \columnwidth instead of \textwidth to defind the width of the figures. It will make the switch from one column to two columns easier. 
A: Indeed, that is a useful point when setting up diagrams and tables, thanks!


TODO: abstract, summary, fill section 3, modify the detail, reference. monitor the farming job and rerun the held ones.


2.8 progress
reference in Introduction and Theoretical ---done!
Observable   ----in doing

2.10 progress
reference in Observable  ---done!
check if higher-order is in ATLAS 2022 eletron pair observation (even not match the lowest one, so wired, but according to the content in that article, I don't think higher-order is in there)
check KaiFeng's measurement of Ru+Ru and Zr+Zr Breit Wheeler process on total cross section, still not HO effects, a dismay trendency...

TODO:  rephrase one paragraph in Observable
review the course



==> summary.tex <==
\section{Summary}
 Due to the large Z of nuclei, the nonpertubative QED should be involved in the description of the experiment measurements of Breit-Wheeler process. But few signs have been presented so far until Zha summarized and calculated most of the available data of total cross section. In this paper, we perform the prediction of lowest order and higher order vacuum lepton pair production in RHIC and LHC collision energies, and qualify the sensitivity of differential cross section, pair transverse momentum and polarization modulation to higher order effects by calculating their correction ratios. Through the QED calculation, we find that the higher order influence on differential cross section become sizable with the large overlap of two nuclear electric field. And for the $\cos 2  \phi$ ($\cos 4 \phi$) modulation and  $\sqrt{\langle P_{T}^2 \rangle }$, their maximum correction ratios appear around the impact parameter of two times the nuclear radius..
 %Besides, an obvious sign transition of the lowest-order $A_{2 \phi}$ is found instead of higher-order calculations, thus the ratio of $A_{2 \phi}$ propose an unprecedentedly sensitive probe to higher order effects. As a series of production activities will be performed at RHIC and LHC in the near future, this work suggests a path to the hidden higher order effects with larger statistics.
Furthermore, our study also present a significant sign transition in the lowest-order $A_{2 \phi}$ instead of higher-order results, which makes it an unprecedentedly sensitive probe to higher-order effects.
A series of future production activities of Au+Au and Pb+Pb collisions are scheduled at RHIC and LHC. This work could outline a path to uncover hidden higher-order effects with larger statistics.

\label{sum}

